Privacy in RFID and mobile objects

Radio Frequency Identification (RFID) is a technology aimed at eficiently identifying and tracking goods and assets. Such identification may be performed without requiring line-of-sight alignment or physical contact between the RFID tag and the RFID reader, whilst tracking is naturally achieved due to the short interrogation field of RFID readers. That is why the reduction in price of the RFID tags has been accompanied with an increasing attention paid to this technology. However, since tags are resource-constrained devices sending identification data wirelessly, designing secure and private RFID identification protocols is a challenging task. This scenario is even more complex when scalability must be met by those protocols. Assuming the existence of a lightweight, secure, private and scalable RFID identification protocol, there exist other concerns surrounding the RFID technology. Some of them arise from the technology itself, such as distance checking, but others are related to the potential of RFID systems to gather huge amount of tracking data. Publishing and mining such moving objects data is essential to improve efficiency of supervisory control, assets management and localisation, transportation, etc. However, obvious privacy threats arise if an individual can be linked with some of those published trajectories. The present dissertation contributes to the design of algorithms and protocols aimed at dealing with the issues explained above. First, we propose a set of protocols and heuristics based on a distributed architecture that improve the efficiency of the identification process without compromising privacy or security. Moreover, we present a novel distance-bounding protocol based on graphs that is extremely low-resource consuming. Finally, we present two trajectory anonymisation methods aimed at preserving the individuals' privacy when their trajectories are released.

==> Chapter3.tex <==
\section{Security, Privacy, and Scalability Issues on RFID Identification Protocols}

The rapid proliferation of RFID solutions strongly supports the vision of
ubiquitous computing, in which tags interacting with readers throughout our
everyday life improve our experiences with the environment. Consequently,
in most applications, readers must be able to identify one or several tags among
a set of millions or billions. This scenario characterises an important property that an RFID identification
protocol should meet; scalability.

As for most identification systems, being secure and private are another two mandatory properties of RFID systems. These two features are even more relevant in the RFID context due to the insecure and easily accessible communication channel between tags and readers. Generally speaking, security means that data stored in a tag's memory should be accessed only by authorised parties and that impersonating or counterfeiting a tag may be achieved just with a negligible probability. On the other hand, privacy-preservation may be defined as the ability of tags to generate uncorrelated identification messages.


\subsection{Security}

RFID systems are subject to plenty of attacks, from attacks operating on the physical layer to attacks exploiting weaknesses on those protocols executed at the application layer~\cite{DBLP:journals/isf/MitrokotsaRT10, DBLP:conf/iwrt/MitrokotsaRT08, springerlink:10.1007/11599548_7}. Physical attacks may be as simple as wrapping an RFID tag in aluminum foil, which potentially causes denial of services (DoS) because readers will be not able to communicate with such a tag. Other physical attacks are more sophisticated (\emph{e.g.} jamming attacks that permanently damage radio devices
or side-channel attacks that obtain information from the physical implementation of cryptosystems). However, in the present dissertation, we focus on adversaries aimed at breaking the identification/authentication schemes by using theoretical weaknesses of such algorithms. To do so, we assume that the adversary can observe, block, modify, and inject messages in the communication between a tag and a reader. Furthermore, as tags are not tamper-resistant, we assume an adversary able to clone and tamper with any RFID tag.

The most relevant attack to RFID systems is the so-called \emph{spoofing} or \emph{impersonation} attack. In this attack, an adversary is able to clone a tag without physically replicating it. By doing so, the adversary gains the privileges of such tag, which is considered an important security threat for almost every RFID applications. The worst situation occurs when the adversary is able to break the cyptosystem used during the authentication process (\emph{total break}), \emph{i.e.} the adversary has knowledge of the authentication protocols and the secrets. In other cases, the adversary does not even need to spend too much time breaking the authentication protocol. In contrast, the adversary could impersonate a tag by replaying and/or manipulating some tag's responses recorded from past transactions (\emph{forgery}). Although these attacks have been successfully coped by lightweight and symmetric key cryptography suitable for low-cost RFID tags~\cite{WeisSRE-2003-spc}, there still exist open issues when privacy and scalability must be also considered.



\subsection{Privacy}

There exist two main privacy concerns in RFID systems: information leakage and traceability. Information leakage is potentially dangerous because tags may reveal sensitive information about products (\emph{e.g.} the name of drugs or the price of expensive products). Such data may be used for quick, easy, and low-cost profiling of individuals, or even for industrial espionage. The basic idea to prevent information leakage in RFID systems is to move all the tags' data to one or several servers. By doing so, only authorised parties may retrieve those data when required. However, this may not prevent traceability. For instance, a tag sending its unique identifier does not reveal trivial information about the object to which is attached, but it is traceable. To thwart traceability, readers and tags should exchange \emph{fresh} information at each identification so as to make two different tag's response \emph{indistinguishable}.

The challenge is that indistinguishability is an application dependant concept where adversaries' abilities, tag's owners, physical constrains, etc., must be taken into account in order to provide a fair privacy definition for RFID systems. That is why different privacy models for RFID have been defined~\cite{Ng:2008:RPM:1462455.1462478, springerlink:10.1007/978-3-540-88313-5-18, Avoine-2005-techrep, Vaudenay:2007:PMR:1781454.1781461, Le07forward-securerfid}. Among them, we recall two well-known notions of privacy proposed by Avoine in~\cite{Avoine-2005-techrep}:

\begin{definition}[Universal untraceability]\label{def:universal}
Universal untraceability is achieved when any pair of tag's responses, separated by a successfully identification with a legitimate reader, cannot be correlated with high confidence by an adversary.
\end{definition}

\begin{definition}[Existential untraceability]\label{def:existential}
Existential untraceability is achieved when any pair of tag's responses cannot be correlated with high confidence by an adversary.
\end{definition}

Intuitively, existential untraceability is stronger than universal untraceability. Note that, the latter ensures privacy against passive adversaries only. That is why, protocols that achieve universal untraceability are usually referred as \emph{passively private}, whilst those protocols achieving existential untraceability are referred as \emph{actively private}~\cite{DBLP:journals/comcom/AlomairP10}.

There exist other notions of privacy in RFID systems namely, forward and backward untraceability. Both notions rely on the fact that RFID tags are not tamper-resistant and thus, an adversary may be able to get full access to the internal state of a tag. Informally, backward and forward untraceability ensure that revealing the internal state of a tag cannot help an adversary to identify previous or future transactions of such tag. However, both are beyond the scope of this dissertation (Interested readers may refer to~\cite{Berbain:2009:EFP:1653662.1653669, springerlink:10.1007/s11277-010-0001-0, 4144831, Song:2008:RAP:1352533.1352556, Cai:2009:AIR:1514274.1514282, 4815081, springerlink:10.1007/s11277-010-0001-0, Berbain:2009:EFP:1653662.1653669, Le07forward-securerfid}).

\subsection{Why is secure, private, and scalable identification hard?}

An RFID identification system where tags send their unique identifier in plain text to readers is scalable (\emph{e.g.} EPC Radio Frequency Identity Protocols Class-1 Generation-2 UHF	RFID~\cite{epcglobal, class_1_gen_2}). In some way, this is how the barcode systems work. However, from the security point of view, it would be quite easy to counterfeit an RFID tag just by building a device able to replay the unique identifier of this tag, which was previously eavesdropped or maybe read from the tag's embodiment. Some RFID manufacturers argue that, in any case, counterfeiting an RFID tag is much more difficult than counterfeiting a barcode label. Actually, this is true for RFID tags intended as the replacement of barcode labels. But RFID systems aimed at being an active part of the future of pervasive computing need anti-counterfeiting measures; they need entity authentication~\cite{Menezes:1996:HAC:548089}.

Public key cryptography (PKC) is known to achieve private and scalable authentication. Actually, most of the applications we nowadays use are protected by PKCs, namely secure remote login (SSH), digital signatures, internet key exchange (IKE), digital cash and secure transparent voting. That is why so many efforts have been devoted to designing and implementing asymmetric cryptosystems
such as Elliptic Curve Cryptosystem (ECC)~\cite{Batina07public-keycryptography} and N-th Degree Truncated Polynomial Ring (NTRU)~\cite{springerlink:10.1007/3-540-36563-X_9}, in RFID tags. However, they require a high number of logic gates to be implemented in tags. Therefore, the price of tags
will increase drastically to accommodate those cryptosystems in RFID tags. Even though other proposals~\cite{Girault_thefeasibility, springerlink:10.1007/11967668_24} reduce the number of required logic gates by performing some pre-computation and storing partial results in tags, they increase the memory usage to around 1700 bits. It is an open problem whether public key cryptography will be suitable for low-cost RFID tags. Therefore, most RFID identification protocols are based on symmetric key cryptography rather than on public key cryptography.

However, symmetric key cryptography does not satisfy all the requirements of RFID systems because, in general, it
draws scalability problems in the server's side. Since tags are not tamper-resistant, each tag must contain a unique and private key with which encrypt its response. The paradox is that, in order to determine the tag's identity the server needs to decrypt the message using the tag's key, but retrieving the tag's key is only possible when the server knows the tag's identity. Consequently, the server should perform an exhaustive search looking for the proper key to decrypt the message. Several protocols overcome this scalability problem by performing an update phase after the identification process (Stateful protocols)~\cite{NingLY-2011-cje, AlomairLP-2010-jcs, Li:2007:PRC:1229285.1229318, 4912773, springerlink:10.1007/11601494_13, ChatmonVB-2006-techrep, Ateniese:2005:URT:1102120.1102134, Karthikeyan:2005:RSW:1102219.1102229}. This means that the tag and the reader should share and synchronously update the next identification message. However, it has been shown~\cite{YuSMS-2009-esorics} that this synchronization process must be carefully designed in order to resist Denial of Services attacks. On the other hand,
 the update phase is not only useless against active adversaries, but also is rather inefficient in the tag's side. Note that, a write operation in a tag may take roughly $16.7$ milliseconds, while a read operation around $0.007$ milliseconds~\cite{5678437}. Indeed, writing in the tag's memory is a time consuming operation; roughly five times more time consuming than a classical AES-128 encryption, which needs around $2.8$ milliseconds.

In conclusion, three main techniques have been proposed for the private identification of RFID tags: (i) Public key cryptosystems that are secure, private, and scalable, but not suitable for low-cost tags. (ii)  Stateful protocols which are scalable, but they are not strong against active attacks and may be less efficient than other symmetric key protocols due to the writing operation in the memory of the tags. (iii) Stateless protocols based on symmetric key cryptography that could be lightweight, private, and secure, but not scalable. As a result, designing lightweight, secure, private, yet scalable, RFID identification protocols still is a challenging task.

\subsection{Advances in RFID identification protocols}

As stated in~\cite{Chien-2007-ieeetdsc}, a tag can be classified according to the operations it supports. \emph{High-cost} tags are those that support on-board conventional cryptography like symmetric encryption and public key cryptography. In turn, \emph{simple} tags are also considered high-cost tags, but they only support random number generators and one-way hash functions. Likewise, low-cost tags can be classified as \emph{lightweight} tags or \emph{ultralightweight} tags. Both, are able to compute simple bitwise operations like XOR, AND, OR, etc, but the former also support a random number generator (RNG) and simple functions like a cyclic redundancy code (CRC) checksum. Undoubtedly, low-cost and simple tags, intended as the replacement of the barcode labels, represent the greatest challenge in terms of security and privacy preservation.

\subsubsection{Identification protocols for low-cost tags}

Several efforts have been made in order to achieve some level of security in low-cost tags~\cite{Wong:2006:CAR:1143147.1143152, citeulike:1141061, Burmester:2008:SEG:1788857.1788887}. One of the first proposals in this direction is due to Duc et. al.~\cite{citeulike:1141061}. They designed a protocol where messages are encrypted using a CRC-16 function and randomized by an updating key process. Although this protocol is not resilient to desynchronization attacks~\cite{Chien:2007:MAP:1222669.1222985}, its main weakness relies in the linearity of the CRC-16 function. Indeed, Burmester and Medeiros~\cite{Burmester:2008:SEG:1788857.1788887} show how to successfully implement an impersonation attack by eavesdropping only one session of the protocol. In the same article, four protocols with different levels of privacy are proposed. The first encrypts messages using the RNG defined in the EPCGlobal2 standard seeded with a key shared by the tag and the reader. The security of this protocol is based on the statistical behavior of the RNG. However, the key is of size 16 bits therefore an exhaustive search on all possible $2^{16}$ key values can be enough to recover the key. On the other hand, EPCGen2 does not specify any protection of the RNG against the \emph{related-key} attack, in which it is possible to find a correlation between a sequence of outputs given by the RNG defined in the EPCGlobal2~\cite{Burmester:2008:SEG:1788857.1788887}. Therefore, an adversary could be able to disambiguate tags that respond with pseudonyms drawn from a EPCGlobal2 RNG complaint. The solution proposed in~\cite{Burmester:2008:SEG:1788857.1788887} is to build a Pseudo Random Function (PRF) from a RNG~\cite{DBLP:journals/jacm/GoldreichGM86}. The new PRF has an input size of 32 bits and it is defined by recursively executing a RNG 16 times.

%%Among the protocols defined in ~\cite{Burmester:2008:SEG:1788857.1788887}, the first three of them are not scalable, while the last one relies on an update process.

Other proposals do not even consider tags generating random numbers. In such protocols, the randomness in the tag's side is provided by readers. It should be noted that, those type of protocols either do not provide anonymity or ensure privacy by updating tags' internal state. In 2006, the first three of ultralightweight protocols were proposed: M$^{\mbox{2}}$AP~\cite{DBLP:conf/uic/Peris-LopezCER06}, EMAP~\cite{Peris-lopez06emap:an} and LMAP~\cite{PerisHER-2006-rfidsec}. Although it was a step forward on the security of low-cost tags, and many other ultralightweight protocols~\cite{Burmester:2008:SEG:1788857.1788887, Peris-Lopez:2009:AUC:1530270.1530277, Chien-2007-ieeetdsc} have been proposed so far, all of them have been proven to be insecure~\cite{YehL-2010-iasl, AvoineCM-2010-rfidsec, HernandezEPQ-2009-wcc, Phan-2008-ieeetdsc, 4159809, Li07securityanalysis}. According to Peris-Lopez et. al.~\cite{Peris-Lopez:2009:AUC:1530270.1530277}, the main weakness of these protocols is the use of triangular functions like AND, XOR, etc. This problem was detected by Chien~\cite{Chien-2007-ieeetdsc} thus, he incorporated a left rotation operation (which is non triangular) to his proposal named SASI. Nevertheless, the SASI protocol has other weaknesses that can be found in~\cite{AvoineCM-2010-rfidsec, Phan-2008-ieeetdsc, HernandezEPQ-2009-wcc, Peris-Lopez:2009:AUC:1530270.1530277}. As a consequence, Peris-Lopez et. al. designed the Gossamer protocol~\cite{Peris-Lopez:2009:AUC:1530270.1530277} aimed at being more secure than previous ultralightweight protocols, though more computationally expensive. In a similar line, Juels proposed a protocol~\cite{Juels03minimalistcryptography} where each tag has a list of one-time pads that together with the tag's keys identify the tag. The protocol is minimalist in the sense that involves only low-cost operations like: rudimentary memory management, string comparisons, and a basic XOR. However, the security of this protocol depends on the size of a list that should be updated at each session.

A completely different approach to the security of RFID systems was proposed by Juels in~\cite{springerlink:10.1007/11535218}. Juels adopts the human-to-computer authentication protocol designed
by Hopper and Blum (HB)~\cite{Hopper01asecure}, and shows it can be practical for low-cost
pervasive devices. HB is a probabilistic protocol consisting of several rounds (around 128 according to Hopper and Blum~\cite{Hopper01asecure}). In each round, the verifier sends $n$-bit of challenge and the prover responds correctly to each bit with a probability greater than $1/2$. At the end of the protocol, the verifier decides whether the prover gave an enough number of correct bits of response. The HB protocol can be also considered an ultralightweight protocol. Later, Juels modified slightly the HB protocol proposing a new protocol~\cite{springerlink:10.1007/11535218} (HB$^+$) that claims to be secure against active adversaries. Although HB$^+$ is suitable for EPC-Gen 2 tags, it has
a high false rejection rate (for 80 bits of security, the false rejection rate is estimated
at $44\%$~\cite{DBLP:conf/eurocrypt/GilbertRS08, cryptoeprint:2005:237}). Furthermore, the communication overheads increase linearly with the security parameter, which may be chosen around the $80$ bits~\cite{Fossorier06anovel}. Another protocol based on an NP-complete problem was proposed by Castellucia and Soos~\cite{CastelluscciaS-2007-rfidsec} at RFIDSec'07. Their protocol (ProbIP) is based on the hardness of the boolean satisfiability problem (SAT), which is proven to be in the NP class of complexity. However, the protocol is neither private nor secure as was shown in~\cite{Ouafi:2008:PRR:1788494.1788513}.

A recent proposal \cite{Wu:2009:HSR:1574927.1574959} based on the hardness of the \emph{noisy polynomial interpolation} problem aims to be private and scalable. However, this protocol presents some shortcomings: i) it has been shown in~\cite{Bleichenbacher:2000:NPI:1756169.1756175} that the \emph{noisy polynomial interpolation} problem can be more easy than expected, ii) the server needs to solve $mb$ polynomials of degree k where m, b, and k, are predefined security parameters and, considering that typical values for m and b are 16 and 8 respectively \cite{Wu:2009:HSR:1574927.1574959}, then, the server needs to solve around 128 polynomials which can be considered still too heavy, iii) finally, tags should be designed with about 10,000 gates more than regular tags capable of hashing computation.

\subsubsection{Identification protocols for simple tags}

In general, lightweight RFID identification protocols use a pseudo random number generator and a symmetric key cryptographic primitive in the tag's side (\emph{e.g.} a hash function or some lightweight block cipher). In this vein, the first AES implementation devoted to RFID tags was proposed in 2004~\cite{FeldhoferDW-2004-ches, FeldhoferWR-2005-ieeproceedings} (Other cryptographic primitives may be found in~\cite{4253019}). However, this implementations require no less than 3400 logic gates, which is beyond the capabilities of extremely constrained devices such as RFID tags~\cite{DBLP:conf/ifip6-8/Peris-LopezHER06}. That is why, several other attempts have been made in order to find cryptographic primitives designed specifically for low-cost RFID tags. To the best of our knowledge, one of the most relevant block ciphers dedicated to RFID tags is PRESENT~\cite{Rolfes:2008:UIS:1430796.1430803, BogdanovKLPPRSV-2007-ches}. Surprisingly, PRESENT only requires between 1000 and 1600 logic gates depending on its variants. Undoubtedly, this improvement supports the rapidly proliferation of RFID identification protocols based on symmetric key cryptography. Nevertheless, even considering that those protocols are suitable for very resource-constrained RFID tags, they should face the scalability issues inherent to these type of proposals. Next, we discuss some of those proposals according to their time complexity in the server's side.

\subsubsection{Lightweight protocols with linear time complexity}

The Improved Randomize
Hash-lock Scheme~\cite{JuelsW-2007-percom, Juels:2009:DSP:1609956.1609963} is a popular RFID identification protocol due to its strong
privacy and security properties at a low cost; only uses a pseudo-random function
generator and a hash function in the tag's side. This protocol works as follows:
The reader sends a random nonce $r_1$ to the tag. Upon reception, the tag
generates a nonce $r_2$ and computes the response $r = h(r_1, r_2, ID)$ where $ID$
is its identifier and $h(...)$ is a one-way hash function. Finally, the reader
receives both, the response $r$ and the nonce $r_2$, with which it performs an
exhaustive search on its database looking for an identifier $ID_i$ such that
$r = h(r_1, r_2, ID_i)$. Figure~\ref{fig:irhl} shows a detailed description of this protocol.
Although the improved randomized hash-lock scheme~\cite{JuelsW-2007-percom, Juels:2009:DSP:1609956.1609963} is a private,
and secure, RFID authentication protocol, it is not acceptable when a large
number of tags should be managed (\emph{e.g.} manufacturing processes). Note that, this protocol performs an exhaustive search on the database in order to identify a tag. That is why, several other protocols based on hash functions have been proposed in order to reduce this linear time complexity.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[tb]\centering
%\small
\scalebox{0.8}{
\begin{tabular}{|ccr|}
\hline
%&& \\
\textbf{Reader (R)}&&\textbf{Tag (T)}\\
\hline
Generates $r_1$ & $\hspace*{1cm}$ $\xrightarrow{\ \ r_1 \ \ }$&\\
& &	Generates $r_2$ \\
& $\hspace*{1cm}$ $\xleftarrow{\ \ r \ \ }$& $r=(r_2, h(r_1||r_2||ID_T))$\\
\multicolumn{3}{|l|}{Computes $r^{T_i}$}\\
\multicolumn{3}{|l|}{$r^{T_i}=(r_2, h(r_1||r_2||ID_{T_i}))$}\\
\multicolumn{3}{|l|}{Identifies $T$ as $T_i$ when $r^{T_i}=r$}\\
\hline
\end{tabular}
}
\caption{Scheme of the Improved Randomized Hash-locks Protocol}\label{fig:irhl}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Another hash-based protocol was proposed by Ohkubo et. al.~\cite{Koutarou03cryptographicapproach}. This protocol uses hash-chains in order to guarantee forward secrecy. However, a high memory consumption
and a linear time complexity $O(N)$ are the main drawbacks of this protocol. Although, Avoine
et. al.~\cite{DBLP:conf/sacrypt/AvoineDO05, Avoine05ascalable} reduce this time complexity to $O(N^{2/3})$ applying a time-memory
trade-off, their improvement demands even more memory on the database than the original protocol~\cite{Koutarou03cryptographicapproach}. Another protocol based on hash-chains and resistant to Denial of Service attacks (DoS) is proposed in~\cite{4144831}. This protocol also achieves forward secrecy, but it presents some privacy issues as shown in~\cite{Ouafi:2008:PRR:1788494.1788513}.

In order to increase efficiency and reduce resource requirements, some protocols use a counter instead of a pseudo-random number generator in the tag's side~\cite{Choi05efficientrfid}. By this technique, tags may dedicate more logic gates to the encryption function and privacy could be guaranteed without updating the key material. However, this type of protocols may be vulnerable to impersonation attacks~\cite{springerlink:10.1007/11807964_27}.


\subsubsection{Lightweight protocols with logarithmic time complexity}

When looking for scalability, the tree-based protocol proposed by Molnar
and Wagner~\cite{Molnar:2004:PSL:1030083.1030112} is considered a secure and highly scalable protocol. It achieves a time complexity in the identification process of $O(b \log^N_b)$ where $N$ is the number of tags and $b$ is the branching factor of the
tree used to store the tag's identifiers. The idea is that each tag in the system is represented by a unique path in the tree, which is simply defined as a sequence of nodes. Then, each tag $T_i$ contains a unique secret key $k_i$ and also contains the keys of the nodes that represent its path in the tree; see Figure~\ref{fig:tree1}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!ht]
  \begin{center}
     \includegraphics{tree1}
  \end{center}
  \caption{A tree of depth 3 and branching factor 2. Tag $T_i$ is represented by the path $k_1^1, k_2^2$ and by its unique and secret key $k_i$.}
  \label{fig:tree1}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Undoubtedly, the unique secret key of each tag is enough to identify it as the improved randomized hash lock~\cite{JuelsW-2007-percom, Juels:2009:DSP:1609956.1609963} does. However, the tree-based protocol uses the path's keys in order to rapidly discard large sets of tags which keys do not match with the received response. It may do so because tags allow readers to check their paths from the root to the leaf. Consequently, assuming that a reader knows a sub-path that matches with the tag's response, it may discard all those tags that do not match with this sub-path. However, since tags share sub-paths and hence they share keys, compromising some tags is enough to trace other tags in the system~\cite{DBLP:conf/sacrypt/AvoineDO05, Nohl06quantifyinginformation}. Although, a trade-off between privacy and efficiency may be achieved considering the privacy measure proposed in~\cite{DBLP:conf/sec/NohlE08}, the tree-based protocols are considered not-private.

There exist some other tree-based protocols aimed at being resistant to the compromising attack~\cite{LuLHHN-2007-percom, 10.1109/SITIS.2007.51}. However, both use an update phase in order to change the tag's keys in each successful execution of the protocol. As have shown above, protocols based on updating the key material do not need complex structures, like trees, in order to be scalable. Furthermore, as shown in~\cite{10.1109/SITIS.2007.51}, synchronizing keys that are shared by several tags is challenging.

\subsubsection{Lightweight protocols with sub-linear time complexity}

A similar idea to the tree-based protocols are the group-based protocols~\cite{4351808}. In these protocols each
tag belongs to a group and has two keys: a group key ($GK$) and an identification
key ($IDK$). Once the tag receives a nonce $r_1$ from the reader, it generates another nonce $r_2$ and sends back $E_{GK}(r_1, r_2, ID)$ and $E_{IDK}(r_1, r_2)$, where $E$ is a symmetric key encryption function and $ID$ is the tag's identifier. The server iterates over all the group's keys until the decryption of $E_{GK}(r_1, r_2, ID)$ successes. If so, it recovers $ID$ and then it just needs to check the decryption of $E_{IDK}(r_1, r_2)$. Note that, the time complexity of this protocol is not linear, but sub-linear\footnote{Theoretically, $f(n)$ is sub-linear if $\lim_{n \rightarrow \infty}\frac{f(n)}{n} = 0$. Nevertheless, at the present thesis we consider that sub-linear time complexity holds if $\frac{f(n)}{n}$ is small enough.}: $O(\frac{N}{k})$ where $k$ is the number of tags in each group. However, if a tag $T$ is compromised by an attacker, she will be able to recover the identity of
every tag belonging to the group of $T$ just by using the group key.

Another type of group-based protocol was proposed in~\cite{CheonHT-2009-eprint}. However, this protocol is different in the sense that a ``meet-in-the-middle'' strategy is used to efficiently identify tags. By this strategy, they reduce the reader computation to $O(\sqrt{N}\log{N})$, which may be considered sub-linear. However, neither this protocol is resistant to compromising attacks.

In the context of using multiple readers (connected to a centralised back-end),
Fouladgar and Afifi~\cite{Fouladgar:2008:SPP:1461464.1461467} point out that, in many
applications, tags are usually queried by the same set of readers. Therefore,
they propose to cluster tags according to the readers that identify them more
often. This idea improves the group-based proposals in the sense that tags are
not randomly assigned to groups, but intelligently clustered according to the
spacial location of the readers that identify them. By doing so, when a reader
receives a tag's response, it first performs a search in the group of tags that
it usually identifies. If it does not success, an exhaustive search is performed
over the whole set of tags' identifiers. The problem of this proposal is that
tags may have a long life-cycle and move through a wide variety of readers. In
this scenario, the protocol could not scale as well as expected.

\subsubsection{Lightweight protocols with constant time complexity}

Privacy-preserving RFID identification protocols with constant time complexity are based, in general, on synchronization between tags and readers. The idea is that any response coming from a legitimate tag is somehow expected by the reader. However, in order to preserve privacy, all the responses might be \emph{fresh} at each session. Therefore, at some point, tags should update their key material or renew their next responses. At the same time, the reader must be sure whether and how the tag updated its internal state. Otherwise, the reader should be provided with a mechanism to identify legitimate tags even when their internal states are unknown or unexpected~\cite{YuSMS-2009-esorics}. Note that, this \emph{desynchronization} between tags and readers could easily occur due to communication failures or active attacks to the protocol.

The basic idea to keep a tag and a server synchronized is to design a mutual authentication protocol so that both update the key material once they have mutually authenticated~\cite{1607559, 1276922, Avoine:2005, Chien:2007:MAP:1222669.1222985, Burmester:2008:ARA:1457161.1457162, citeulike:2632811}. In any case, the server should keep the last correct key used by every tag in order to resist desynchronization attacks. The problem with this approach is that tags are traceable in isolated environments, \emph{i.e.} as long as a tag has not being identified by a legitimate reader, it will send the same response to any reader's interrogation. Note that, this type of protocols are passively private only (see Definition~\ref{def:universal}).

To tackle this problem, some protocols consider the scalability and privacy issues as a matter of agreement between tags and readers~\cite{5318888, 6014260}. This means that a reader is able to identify a tag in constant time only if it was the last who interrogated such tag. Otherwise, the tag's response looks random for the reader and thus, the tag cannot be identified in constant time. Therefore, this type of protocols are actively private (See Definition~\ref{def:existential}), but they are not \emph{unconditionally} scalable.

Both passively and actively private approaches may be improved by pre-computing more than one future tag's responses~\cite{LimKwo06}. Typically, in these approaches tag's responses are based on hash chains~\cite{6014260, FernandezCV-2010-setop}. Then, the server may efficiently identify a tag because it had stored \emph{enough} values of the hash chain used by this tag. Therefore, increasing memory requirements on tags and server both privacy and scalability may be improved. However, it should be noticed that the improvement is achieved by demanding more of a resource that is already quite constrained on tags and servers~\cite{Palmer-2011}.


\subsubsection{Identification protocols for high-cost tags}

High-cost tags are similar to smart-cards. They are far more expensive than low-cost RFID tags, which could drop prices until $0.05 \$$. Nevertheless, there exist some applications requiring a high level of security and privacy in which high-cost tags are not only appropriate, but recommended (\emph{e.g.} passports or toll payment).

In such tags, there exists the possibility of implementing some public key cryptosystems. Especially those requiring less computational capabilities on tags, namely Elliptic Curve Cryptosystem (ECC) or Lattice Based Cryptosystem. A typical ECC implementation could need more than 30K logic gates~\cite{springerlink:10.1007/978-3-540-74442-9_30}, others are able to reduce the computational requirements between 10K and 18K logic gates~\cite{Kumar06arestandards, Hein:2009:ERR:1616707.1616744}, though.

In general, the reduction of computational requirements is achieved by optimizing, manipulating, or removing some operations of the original proposal~\cite{1987}. The idea is to reduce as much as possible the computational requirements of public key cryptosystems while guaranteing security and privacy. However, as shown in~\cite{Bringer:2008:CER:1485310.1485324}, the task could be challenging. In a nutshell, they show that previous ECC proposals for RFID systems~\cite{4519370, 4911179} may be vulnerable to tracking and impersonation attacks.

Other approaches perform some pre-computation in order to reduce the computational overhead in the tag's side. In~\cite{Oren:2009:LPI:1514274.1514283}, Oren and Feldhofer improve the Shamir's public key scheme~\cite{1994-2756} by replacing a pseudo-random sequence of 260 bytes long, by a reversible
stream cipher of less than 300 bits long. Another trade-off between efficiency and memory is shown by Hoffstein et. al. in~\cite{springerlink:10.1007/3-540-36563-X_9}. They propose a lattice based cryptosystem referred as NTRU, which claims to be faster than ECC during the signature and verification processes.

The well-known randomized Rabin encryption scheme has been also adapted to fit the RFID requirements~\cite{OrenF-2008-rfidsec}. Even though this protocol initially had some shortcomings, it was later improved in~\cite{4911191}. Finally, differently to classical public key cryptosystems, a lightweight identification protocol requiring around 3000 logic gates was proposed in~\cite{Kim:2007:RSP:1345530.1345612}. This protocol uses some ECC elements to strengthen RFID security. However, in order to decrease computational demands it does not provide a trapdoor function as usual ECC cryptosystems do. That is why, this approach presents the same scalability problem of other symmetric key cryptosystems.


\subsubsection{Other approaches}

According to the EPC standard, each tag contains a KILL password. A reader knowing the KILL password of a tag is able to disable this tag permanently. Therefore, after the shipping check-out process tags could be ``killed'' in order to preserve the privacy of their holders. Although this measure prevents privacy disclosure, it may not be practical in the long-term because tags cannot be reused. That is why Spiekermann and Berthold proposed a simple scheme so that users are able to disable/enable RFID tags when needed~\cite{springerlink:10.1007/0-387-23462-4_15}. A more sophisticated, yet complex idea, is proposed in~\cite{Engberg04zero-knowledgedevice}. When a tag enters in the post-purchase phase, it supports the ability to change into \emph{privacy mode}. In this mode, tags only accept zero-knowledge proofs from legitimate devices.

There exist other proposals relying on re-encryption in which tags offload most of the computational effort during encryption to the readers or third devices~\cite{Saito04enhancingprivacy, Juels02squealingeuros:, Golle02universalre-encryption}. Those proposals are somehow based on updating the key material in tags. However, they use public key cryptography to re-encrypt the plaintext stored in tags. Therefore, readers knowing the proper private key can obtain the plaintext by decrypting only once, instead of several times as it is usually the case with symmetric key cryptography. Other examples of proposals using a third devices are, RFID guardian~\cite{Rieback05rfidguardian:}, RFID enhancer proxy~\cite{juels:proxies}, noisy tags~\cite{Castelluccia06noisytags:} and, the blocker tag~\cite{Juels03theblocker, JuelsB-2004-wpes}. In addition to those proposals, there exist others proposals based on assumptions not considered by most RFID solutions. In particular, implementation of Physical Unclonable Functions (PUF) on tags have been shown to be useful to cope with the tampering issues of RFID tags~\cite{Tuyls06rfid-tagsfor, Bolotnyy:2007:PUF:1263542.1263714, Bringer:2008:IPT:1432967.1432976}.





==> Chapter3_5.tex <==
\section{Other Issues on RFID Systems}

Tracking and identifying are the main goals of an RFID system. In consequence, those challenges related to the identification process may seem much more relevant than others. However, RFID systems should face many other challenges depending on the application in which they are applied. For instance,  in supply chain management, an RFID tag may change of owner several times. There exist practical situations in which those owners do not trust each other. Therefore, some efforts must be also devoted to the design of \emph{ownership transfer protocols}~\cite{saito2005reassignment}. Furthermore, the proper use of RFID data still is an open issue. Thanks to the RFID technology, individuals' trajectories could be easily collected and released by supermarkets, hospitals, or amusement parks. Thereby, efficient \emph{trajectory anonymization algorithms} are a need for protecting the privacy of RFID users.




\subsection{Ownership transfer}

Let us consider a manufacturer distributing RFID-tagged products to the
point of sale. These products may be sold to buyers who can
resell them to other buyers. Then, in order
to track RFID-tagged products across buyers, they may rely the identification of such tags to some trusted third party (TTP) or they could simply share the identification keys of all tags. However, both solutions have drawbacks. First, it is not always possible for different entities or companies to have a TTP managing their access and privileges to the RFID tags' information. Besides, this solution does not only cause bottlenecks and overloads
on the server side, but also requires readers to be online with the TTP. On the other hand, sharing the tags' identification key among different parties arises trivially privacy issues because previous and future owners of a tag are able to identify it even when it is not in their possession. The idea to tackle this problem relies on {\em ownership transfer processes}, in which tags' keys may be
transferred from previous owners to new owners ensuring
the security and privacy of past and future tag
identifications~\cite{saito2005reassignment}.

%Authorisation recovery
In some special cases, such as for after-sale service of an RFID-tagged object,
the previous owner of a tag might need to temporarily recover the
means of interacting with it. For instance, this happens when the
buyer goes back to the seller to have a guaranteed appliance repaired.
In this case, the current owner of a tag should be able
to transfer its identification rights over a tag to another reader and
to recover the exclusive right of identifying this tag at any moment.
If the reader to whom the identification rights over a tag were
transferred is a previous owner of this tag, the process is
called {\em authorization recovery}~\cite{fouladgar2007efficient},
otherwise the process is called
{\em controlled delegation}~\cite{YuSMS-2010-jcs}.


A great number of authentication/identification protocols for
RFID systems have been proposed in the
literature~\cite{langheinrich2009survey}. However, just a few of
them have been extended to support ownership transfer, authorization
recovery or controlled delegation. When the RFID system supports
ownership transfer, the tags can be used by different owners,
so that they have a longer life cycle. Authorization recovery and
controlled delegation are properties especially designed for
after-sale and maintenance service.

In identification/authentication protocols, RFID systems typically
use a shared key between the tag and the owner's reader.
Since the shared key is only known by the owner's reader,
this reader alone can complete the tag identification successfully.
In ownership transfer protocols there are two players,
the current owner and the future owner. Before the protocol execution,
only the current owner can identify the tag; after the protocol
is completed, only the new owner can identify the tag
successfully. This process is repeated every time
the owner of the tag changes. So far, two assumptions have
been extensively used in order to achieve the property mentioned above:

\begin{itemize}
    \item \textbf{Centralised scheme:} There exists a Trusted
Third Party (TTP) which every entity (owner) trusts.
It is assumed that entities can establish a secure communication.

   \item \textbf{Isolated environment:} There exists a secure environment,
so that each entity can execute the protocol with the tag
without being eavesdropped by an adversary.

\end{itemize}

Both assumptions make sense depending on the application.
A centralised scheme might be used in inventory control
or supply-chain management applications, where all tags are
identified by readers belonging to the same company.
However, when a user buys a product, she does not necessarily trust anyone.
Hence, a centralised scheme is not suitable. In this case, it
is assumed that the user can go to an isolated environment ({\em e.g.}
the user's home), where he can change the tag key without being
eavesdropped by an adversary.

\subsubsection{Ownership transfer model}
\label{otm}
%The ownership transfer protocol allows the secure and private transfer of identification rights over a tag $T$ between two parties. According to~\cite{song2010scalable,YuSMS-2010-jcs}, three different roles in ownership transfer could be defined:
An ownership transfer protocol allows transfering
the rights over a tag $T$ from the current owner to the new owner in a
secure and private way. According to~\cite{song2010scalable,YuSMS-2010-jcs},
there are three different roles (entities) in an ownership transfer protocol:

\begin{itemize}

  \item \emph{The previous owner.} In the past, this entity had the
  ability to identify or track $T$ as much as he wanted,
  but now she cannot perform these operations anymore.

  \item \emph{The current owner.} At the present time, only this entity
  can identify and track $T$.

  \item \emph{The new owner.} She cannot identify or track $T$ at
  the beginning of the protocol. When the protocol finishes,
  $T$ can only be identified or tracked by this entity.
  % but is the actor whom $T$ will be transferred to in order to play the future role of the current owner.

\end{itemize}

%When it is required to transfer the ownership of $T$, the current owner and the new owner will run an ownership transfer protocol on $T$. Doing so, $T$'s secrets and $T$'s data will be passed from the current owner to the new owner. However, the owners' roles change. $T$'s current owner becomes the $T$'s previous owner, while $T$'s new owner becomes the $T$'s current owner.
When it is required to transfer the ownership of $T$, the current
owner and the new owner run an ownership transfer protocol on $T$.
The secrets and data stored in $T$ are transferred from the current
owner to the new owner. Thus, roles change. The current owner of $T$
becomes the previous owner of $T$, while the new owner of $T$
becomes the current owner of $T$.

The ownership transfer process motivates the requirements of
authorization recovery and controlled delegation mentioned
above.
%JOSEP. This has been said in the introduction and the comment
%about scalability issues is unclearly explained.
%
%Authorization recovery is especially designed for after-sale
%service while controlled delegation is a generalization of the
%former with a wide range of applications, {\em e.g.}
%mitigating scalability issues~\cite{fouladgar2007efficient}.
%JOSEP. This below
%repeats things said in the introduction. So I've suppressed it.
%
%By controlled delegation, a current owner is able to give identification rights over a tag to anyone without defeating the ownership of the tag. On the other hand, by authorization recovery, a current owner can give identification rights over a tag just to a previous owner of this tag. In both requirements, the identification rights should be limited.
%For an RFID protocol complying  with ownership transfer, authorization recovery, or controlled delegation, preserving the roles of all the actors is the main requirement. Figure~\ref{fig:system_actors} shows the actors that could be involved in an ownership transfer protocol.
%The roles preservation for all involved actors is the main requirement for an RFID protocol, that complies  with the ownership transfer, the authorization recovery, or the controlled delegation.
Figure~\ref{fig:system_actors} shows the players
that can be involved in an ownership transfer protocol.

\begin{figure}[!ht]
  \centering
   \includegraphics[scale=0.46]{figures/system_environment}
  \caption{A generic scenario for ownership transfer.}
  \label{fig:system_actors}
\end{figure}


\subsubsection{RFID ownership transfer protocols}

%Centralized server TTP
The first solution to the ownership transfer problem based on a
centralised scheme was proposed by Saito et. al.
in~\cite{saito2005reassignment}. In this protocol, tags
receive encrypted messages using the TTP key ($K_{TTP}$).
Since all tags know $K_{TTP}$, they are able to correctly decrypt
the messages coming from the trusted third party. However, tags are
not tamper-resistant and, hence, tampering just one
tag is enough to break the security of the whole system by
finding $K_{TTP}$. Saito {\em et al.}~\cite{saito2005reassignment} also
consider the case where a centralised scheme cannot be used.
%JOSEP. I define backward channel as the channel from tag to reader
In this case, they assume that the backward channel
(from tag to reader) is unreadable
by adversaries. Therefore, a secure communication between
tags and readers is achieved by the reader encrypting messages using a nonce
%JOSEP. I added "sent by the tag to the reader". Please check that this is true.
%ALBERT. En aquest cas, és al revés. És el reader el que envia el nonce al tag per xifrar el seu id
sent by the reader to the tag
that is refreshed at each session. However, although the range of
the backward channel is shorter than the range
of the forward channel from reader to tag, in general, the backward channel
cannot be considered unreadable to adversaries.

Another centralised scheme for ownership transfer and controlled
delegation is proposed by Molnar et al. in~\cite{molnar2006scalable}.
They use a centralised trusted centre named $TC$ to manage tags' keys
in a tree structure. The delegation property is achieved when the
trusted centre gives a subtree of pseudonyms to a reader.
Using this subtree of pseudonyms, a reader is able to
identify a tag $q$ times where $q$ is the number of leaves
of this subtree.
The keys shared by several tags are a protocol weakness in terms of privacy. Note that, compromising just a few tags quickly decreases the privacy of the whole system~\cite{DBLP:conf/sacrypt/AvoineDO05}.

%Garantia
Unlike Molnar {\em et al.}'s protocol~\cite{molnar2006scalable},
other proposals use a counter into the non-volatile memory of tags in
order to control how many identifications can be done after the execution
of a controlled delegation protocol. The basic idea is that tags
give different responses depending on whether the counter $c$ is
less than some threshold $c_{max}$ or equals $c_{max}$. As shown by
Fouladgar and Afifi~\cite{fouladgar2007efficient}, while $c < c_{max}$
the tag responds using a key known just by the trusted centre and
by the readers (the trusted centre gave rights to the readers previously).
Once the counter reaches its maximum value, the tag encrypts
its responses using a key known just by the trusted centre and hence,
the tag identification is only possible through the trusted server.
However, using a counter on the tag side raises two main issues:
(i) the counter must be in the non-volatile memory of the tag; (ii)
giving rights to more than one reader causes that tag keys to be
shared by several readers. Notice that a reader that knows the
identification key of some tag is able to know where and when this
tag is being identified by any other reader.

Schemes based on a centralised and trusted third party require
readers to be online at each execution of the ownership transfer
protocol. Further, some of the parties involved in the ownership
transfer process may not actually trust the TTP. Thus, there exist some
proposals without a TTP. To the best of our knowledge, the first
decentralised protocol relying on the assumption that owners are
able to change the tag key in an isolated environment was proposed by
Yoon and Yoo~\cite{yoon2008two}. However, this protocol has
security vulnerabilities well described in~\cite{kapoor2009vulnerabilities}.
Under the same assumption, Chen {\em et al.}~\cite{chen2009enhancement}
proposed an improvement of Osaka {\em et al.}'s
scheme~\cite{osaka2007efficient}
through authentication of the reader by the tag before changing
the tag key. Although this protocol guarantees a
successful ownership transfer process, a previous owner can
neither check whether a tag was in its possession nor
can temporarily recover the means of interacting with a tag.

The property of authorization recovery~\cite{song2010scalable} allows
a previous owner of a tag to identify it again.
%The ability of giving to the previous owner of a tag the rights to identify again this tag is known as \.
This property is considered a particular case of delegation and
could be achieved simply restoring the key of the previous owner into the tag.
For instance, Dimitriou~\cite{dimitriou2008rfiddot}  proposes a
simple \emph{tag release} command that restores the manufacture
key of the tag. However, this solution gives authorization
recovery rights just to the tag manufacturer.
Song {\em et al.}~\cite{song2010scalable} solve this drawback in their proposal.
Each tag owner remembers the key of the previous tag owner.
Hence, updating the tag key to the key used by the previous owner
is enough for authorization recovery. Although
both protocols~\cite{song2010scalable,dimitriou2008rfiddot} do not
support controlled delegation, they have the advantage of
not needing a trusted third party.
The recent work in ownership transfer~\cite{YuSMS-2010-jcs}
shows that ownership transfer and controlled delegation are
possible in a decentralised scheme. The authors propose a scheme
that achieves all the desired properties defined so far in ownership transfer.
However, their scheme can be used only in those identification/authentication
protocols where: (i) keys are not updated; or (ii) keys are updated
using Song {\em et al.}'s protocol~\cite{song2010scalable}.
Such a constraint has severe effects on the scalability of the
identification process. Note that, although most identification
protocols with key updating are not private against active adversaries,
they can scale better than protocols without key updating.

\subsection{Trajectory anonymization}

The location of an individual can be determined by different techniques. Possibly, the most conventional and ancestral of these techniques is the visual identification of that individual in some place at some moment. Nowadays, this task is far easier since there is no need for a person monitoring or harassing another person. Instead, several technologies widely adopted worldwide can perform this task for us automatically (\emph{e.g.} surveillance cameras, credit card transactions, RFID identification, among others). In addition, today's pervasiveness of location-aware devices like mobile phones and GPS receivers help companies and governments to easily collect huge amount of information about the movements of people.

Analyzing and mining this type of information, also known as trajectories or spatio-temporal data, might reveal new trends and previously unknown knowledge to be used in traffic, sustainable mobility management, urban planning, supply chain management, etc. By doing so, resources might be optimized and business and government decisions can be solid and well-founded. As a result, it is considered that both companies and citizens profit directly from the publication and analysis of databases of trajectories. However, there are obvious threats to the privacy of individuals if their
trajectories are published in a way which allows re-identification of the
individual behind a trajectory.

\red{A tentative solution to preserver individuals' privacy is de-identification, that is, to remove all the identifying attributes of individuals. However, this is often insufficient to preserve individuals' privacy. Other set of attributes such as age, zip-code, and sex, together with external information, can be used to re-identify the individual behind a record. This type of attributes are called \emph{quasi-identifiers}. As an example in the context of spatio-temporal databases, let we consider a GPS application recording the trajectories of some people. Daily routine indicates that a trajectory is likely to begin at the user's home during the morning ending at the user's work place. These information can be easily linked to a single user, whose identity might be obtained from external source of information like telephone directories or social networks.}
dasfadas


Estimating how much external information is available for an adversary is a challenging task~\cite{kaplan10}. Furthermore, the time information and its relation with the spatial information gives a distinctive nature to the spatio-temporal data over the microdata, \emph{i.e.} over records describing users' data without a sequential order. That is why traditional anonymization and sanitization methods for microdata~\cite{fung10} are not suitable for spatio-temporal data and viceversa. Therefore, specific anonymization algorithms devoted to thwart privacy attacks on published databases of trajectories is an increasing need with each passing day.


\subsubsection{$k$-Anonymity and microaggregation}
\label{micro}

%JOSEP???? Add some 2011 reference

A lot of work has been done in anonymizing microdata
and relational/transactional
databases~\cite{samarati98,sweeney02a,truta06,machanavajjhala06,wong06,li07,nergiz07,domingo08,Zhang07aggregatequery}; see also the recent survey~\cite{fung10}.
A usual goal in anonymization is to achieve
$k$-anonymity~\cite{samarati98,sweeney02a}, which is the ``safety in
numbers'' notion.

Anonymizing a microdata set by mere suppression
of direct identifiers ({\em e.g.}, names, passport numbers)
is not enough to prevent privacy disclosure. Indeed,
other attributes, called quasi-identifier attributes, are often
available in the data set such that their combination
allows re-identifying the individual to whom
a record corresponds: for example, Sweeney~\cite{sweeney} found
that ``87\% of the US population is uniquely identified
by \{date of birth, gender, 5-digit ZIP\}''.
Re-identification allows linking the confidential attributes in
a record ({\em e.g.}, salary or health condition) with a specific individual,
and this constitutes a disclosure.

An anonymized  microdata set is said to satisfy $k$-anonymity if each
combination of quasi-identifier attribute values is shared
by at least $k$ records. Therefore,
this property guarantees that an adversary is unable
to identify the individual to whom an anonymized record
corresponds with probability
higher than $1/k$.

$k$-anonymity cannot be directly achieved with
spatio-temporal data, because any point or time can be regarded as
a quasi-identifier attribute~\cite{abul08}.
Direct $k$-anonymization would require
a set of original trajectories to be transformed into a set of
anonymized trajectories such that each of the latter
is identical to at least $k-1$ other anonymized trajectories.
This would obviously cause a huge information loss.

Generalization was the computational approach
originally proposed to achieve $k$-anonymity~\cite{samarati98,sweeney02a}.
Later, Zhang {\em et al.} introduced
the permutation-based approach~\cite{Zhang07aggregatequery},
that has the advantage of not being constrained by domain
generalization hierarchies. In~\cite{domingo05} it was shown
that $k$-anonymity could also
be achieved through microaggregation of quasi-identifiers.
Microaggregation~\cite{domingo02} works in two stages:
\begin{enumerate}
\item {\em Clustering}. The original records are
partitioned into clusters based
on some similarity measure (some kind of distance)
among the records with the restriction that each
cluster must contain at least $k$ records.
Several microaggregation heuristics are available
in the literature, some yielding fixed-size clusters
all of size $k$, except perhaps one ({\em e.g.} the
MDAV heuristic~\cite{domingo05}), and some yielding
variable-size clusters, of sizes between $k$ and $2k-1$
({\em e.g.} $\mu$-Approx~\cite{muapprox} or V-MDAV~\cite{DBLP:conf/ijcnn/SolanasGM10}).
\item {\em Anonymization}. Each cluster is anonymized individually.
Anonymization of a cluster may be based on an aggregation
operator like the average~\cite{domingo02} or the median~\cite{domingo05},
which is used to compute the cluster centroid; each record in the
cluster is then replaced by the cluster centroid.
Anonymization of a cluster
can also be achieved by replacing the records in the cluster with synthetic
or partially synthetic data; this is called hybrid data
microaggregation~\cite{domingo10a} or condensation~\cite{aggarwal04}.
\end{enumerate}


\subsubsection{Clustering algorithms for trajectories}

Just like in microdata records, suppressing direct identifiers
from trajectories is not enough for privacy~\cite{kaplan08}.
Consequently, several anonymity notions and methods
for trajectories have been
proposed~\cite{hoh05,gruteser05,hoh07,bonchi08,pensa08,bonchi09,abul08,nergiz08,terrovitis08,mohammed09,nergiz09,yarovoy09,monreale10,abul10,hoh10}.
Among those works, we next review the ones that try to achieve some notions of trajectory $k$-anonymity.
Other comparisons of several trajectory anonymization
methods can be found in~\cite{bonchi09,abul10}.


Abul, Bonchi and Nanni proposed a notion of trajectory $k$-anonymity assuming uncertainty on the data provided by technologies like GPS~\cite{abul08,abul10}. They also proposed two methods to achieve privacy according to their notion of privacy. In the
original method --Never Walk Alone (NWA)~\cite{abul08}--,
the set of trajectories is partitioned
into disjoint subsets in which trajectories begin and end at roughly
the same time; then trajectories
within each set are clustered using the Euclidean distance. In the follow-up
method --Wait For Me (W4M)~\cite{abul10}--, the original trajectories are
clustered using the edit distance on real sequences (EDR)~\cite{chen05}.
Both approaches proceed by anonymizing each cluster separately. Two
trajectories $T_1$ and $T_2$ are said to be co-localized
with respect to $\delta$ in
a certain time interval $[t_1,t_n]$ if for each triple $(t, x_1,y_1)$
in $T_1$ and each triple $(t, x_2,y_2)$ in $T_2$
with $t \in [t_1,t_n]$, it holds that
the spatial Euclidean distance between both triples
is not greater than $\delta$.
Anonymity in this context
means that each trajectory is co-localized with at least $k-1$ other
trajectories ($(k,\delta)$-anonymity).
Anonymization is achieved by spatial translation of trajectories inside a
cluster of at least $k$ trajectories having the same time span. In the
special case when $\delta=0$, the method produces one centroid/average
trajectory that represents all trajectories in the cluster.
{\em Ad hoc} preprocessing and outlier removal facilitate the process.
Utility is evaluated in terms of trajectory distortion and impact
on the results of range queries.
The problem with the NWA method is that partitioning the set of all
trajectories into subsets sharing the same time span may produce too
many subsets with too few trajectories inside each of them;
clearly, a subset with less than $k$ trajectories cannot be
$k$-anonymized. Also, setting a value for $\delta$ may be
awkward in many applications ({\em e.g.}
trajectories recorded using RFID technology).

Another $k$-anonymity based notion for trajectories consisting of ranges of
points and ranges of times has been proposed in~\cite{nergiz08}
and~\cite{nergiz09}. It uses clustering to minimize the ``log cost
metric''; which measures the spatial and temporal translations
with user-provided weights.
Minimizing the log cost therefore maximizes utility. The
clusters are anonymized by matching points of the trajectories and
generalizing them into minimum bounding boxes. Unmatched points are
suppressed and so are some trajectories. The anonymized data are not
released; instead, synthetic ``atomic'' trajectories (having
unit x-range, y-range and time range) are
generated by sampling the bounding boxes. This approach
does not release standard trajectories but
only trajectories with unit ranges.

In~\cite{monreale10}, $k$-anonymity means that an original
trajectory $T$ is
generalized into a trajectory $g(T)$ (without the
time information) in such a way that $g(T)$ is
a sub-trajectory of the generalizations
of at least $k-1$ other original trajectories.
Ignoring the time information during anonymization and complex plane
tessellations used to achieve the $k$-anonymity are the main drawbacks of
this method. Utility is measured by comparing clustering results.

%JOSEP. Afegida referencia.
\cite{hu10} is another proposal for achieving $k$-anonymity
of trajectories by means of generalization. The difference
lies in the way generalization is performed: the authors propose
a technique called \emph{local enlargement}, which guarantees that
user locations are enlarged just enough to reach $k$-anonymity,
which improves utility of the anonymized trajectories.

The adapted $k$-anonymity notion for trajectories in~\cite{yarovoy09}
is stated in terms of a bipartite attack
graph relating original and anonymized trajectories such that
the graph is symmetric and the degree of each vertex representing
an anonymized trajectory is at least $k$.
The quasi-identifiers used to define identities are the times of the positions
in a trajectory, and the anonymity is achieved by generalizing points of
trajectories into areas on the grid. An
information loss metric defined for
such areas is used to evaluate the utility of the anonymized data.

Some approaches assume that the data owner anonymizing the database knows
exactly what the adversary's knowledge is. If the adversary is assumed to
know different parts of the trajectories, then those are removed from the
published data~\cite{terrovitis08}. However, this work only considers
sequential place visitation without real time-stamps. If the adversary is
assumed to use some prediction of continuation of a trajectory based on
previous path and speed, then uncertainty-aware path
cloaking~\cite{hoh07,hoh10} can suppress these trajectories; this
procedure however, results in high information loss.

%JOSEP. Afegides referÃ¨ncies palanisamy, hu10tkde
Additional related work about anonymization of spatio-temporal data can be
found in the literature about location privacy, focused on applications
such as privacy-aware location-based services (LBS) or
privacy-aware monitoring
of continuously moving objects. Location privacy
in the LBS-setting was first proposed in~\cite{gruteser03}.
See~\cite{palanisamy11,hu10tkde} for recent papers on location privacy,
in which mobile objects protect the privacy of
their continuous movement. Location
privacy is enforced on individual sensitive locations or unlinked
locations in an on-line mode; often, data are anonymized on a per-request
basis and in the context of obtaining a location-based service.
In this dissertation, we focus on
off-line publishing of whole spatio-temporal databases rather than
protecting specific individuals from LBS providers
or on-line movement monitoring. In general, a solution to location privacy is
not a solution for publishing anonymized trajectories, and vice versa.



==> Chapter6.tex <==
\chapter{A Scalable RFID Authentication Protocol Supporting Ownership Transfer and Controlled Delegation}
\label{chap:6}

\emph{This chapter describes a scalable RFID identification protocol based on update. Thanks to this update feature supported by tags, the proposed protocol is also able to perform ownership transfer, controlled delegation, and authorization recovery processes.}

\minitoc

Preserving privacy among owners is a challenging task when the ownership
of tagged products is transferred between them. Ownership transfer,
authorization recovery and controlled delegation schemes
should be designed to be secure and private not only against
external adversaries, but also against previous owners. In this chapter, a new decentralized
identification protocol with ownership
transfer and controlled delegation is proposed.
On the reader's side, tag identification is scalable in the number of tags.
Once the tag has been identified, its identification key is updated.
This property is used in the ownership transfer process in order
to update the owner's key. Similarly to the
proposals~\cite{molnar2006scalable} and~\cite{song2010scalable},
the protocol has the advantage of supporting controlled delegation without
needing a counter on the tag's side. Also, although it is
based on synchronization, unlike
previous proposals~\cite{YuSMS-2010-jcs,song2010scalable,dimitriou2008rfiddot}, our protocol is still secure and private against active adversaries.



\section{Our proposal}
\label{proposal}


Our protocol is based on the
synchronization between the server and the tag, but even
when these are desynchronized, it still can be scalable and
resistant against denial-of-service attacks.
The protocol has been designed to guarantee that an attacker can not
distinguish whether a tag is synchronized or not. This fact adds one
more degree of difficulty for an attacker who wants to trace a tag or mount
a denial-of-service attack. Together with the above mentioned features,
our proposal supports ownership transfer and controlled delegation
in a decentralized scheme. The result is a secure, private and scalable RFID
identification protocol that supports ownership transfer
and controlled delegation.

Our protocol consists of five phases:
initialization, synchronized identification, desynchronized identification,
update and ownership transfer. The update phase is executed after
each successful identification. If the tag cannot be updated and
the system is desynchronized, it can still be identified by a
desynchronized identification phase that preserves all the
security and privacy properties. Table~\ref{tab:Notacion} summarizes
the notation used to describe the new proposal.

\begin{table}[ht]
\begin{centering}
\caption{Notation used in the protocol}
\label{tab:Notacion}
\begin{tabular}{
>{\raggedright}m{0.2\textwidth}
>{\raggedright}m{0.45\textwidth}}
\toprule
$R$ & Reader\tabularnewline
$T$ & Tag\tabularnewline
$id$ & Tag identifier\tabularnewline
$ik$ & Identification key\tabularnewline
$uk$ & Update key\tabularnewline
$r_{i}$ & Random number\tabularnewline
$h()$ & One-way hash function\tabularnewline
$h_{k}()$ & Keyed hash function (HMAC)\tabularnewline
$PRNG$ & Pseudo-random number generator\tabularnewline
$SYNC$ & Synchronization state\tabularnewline
$C_{i}$ & Pseudo-random bit sequence\tabularnewline
$S$ & Pseudo-random bit sequence\tabularnewline
$m_{i}$ & Update message \tabularnewline
$k_{\delta}$ & Hash chain\tabularnewline
$||$ & Concatenation operator \tabularnewline
$\oplus$ & XOR operator\tabularnewline
\bottomrule
\end{tabular}
\par\end{centering}
\end{table}


\subsection{System environment}

The proposed protocol requires a server that hosts its own database and
readers that transmit information from tags to the server.
For each tag, the server stores a record containing the
following data (see Table~\ref{tab:Tabla-de-valores}):

\begin{itemize}
\item \emph{$id$}: The tag identity.
\item \emph{$Info_{id}$}: The tag information.
\item \emph{$uk$}: An update key $uk$ that only changes after
the execution of a successful ownership transfer protocol.
This key is only known by the current tag owner.
\item \emph{$ik$ and $h_{id}(ik)$}: A tag identification key $ik$ and
its associated hash value $h_{id}(ik)$ using the tag identifier as key. The hash value is used to identify a tag in a lookup table.
\item \emph{$ik_{old}$ and $h_{id}(ik_{old})$}: A previous tag
identification key $ik_{old}$ and its associated hash value
$h_{id}(ik_{old})$ are kept in order to prevent denial-of-service attacks.
\item \emph{$Table\, k$}: A table used to identify a tag in case
of desynchronization between the tag and the server. Row 1 and row 2
in the table store hash chains of size $MAX$ starting
from $ik_{old}$ and $ik$, respectively.
\end{itemize}

\begin{table}[ht]
\begin{centering}
\caption{DB values for each tag}
\label{tab:Tabla-de-valores}
\begin{tabular}{>{\centering}m{4cm}>{\centering}p{6cm}}
\toprule
Tag data & $Table\, k$ \tabularnewline
\hline
\begin{tabular}{c}
$id$\tabularnewline
$Info_{id}$\tabularnewline
$uk$\tabularnewline
$ik$\tabularnewline
$h_{id}(ik)$\tabularnewline
$ik_{old}$\tabularnewline
$h_{id}(ik_{old})$\tabularnewline

\end{tabular} &
\begin{tabular}{c|c|c|}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{$k_{i}^{old}$} & \multicolumn{1}{c}{$k_{i}$}\tabularnewline
\cline{2-3}
0 & $h_{id}(ik_{old})$ & $h_{id}(ik)$\tabularnewline
\cline{2-3}
1 & $h_{uk}(k_{0}^{old}||id)$ & $h_{uk}(k_{0}||id)$\tabularnewline
\cline{2-3}
2 & $h_{uk}(k_{1}^{old}||id)$ & $h_{uk}(k_{1}||id)$\tabularnewline
\cline{2-3}
\vdots & \vdots & \vdots \tabularnewline
\cline{2-3}
$MAX$ & $h_{uk}(k_{MAX-1}^{old}||id)$ & $h_{uk}(k_{MAX-1}||id)$\tabularnewline
\cline{2-3}
\end{tabular}
\tabularnewline
\bottomrule
\end{tabular}
\par\end{centering}
\end{table}

\subsection{Protocol phases}

In this section we describe the seven different phases of our protocol: (i) initialization, (ii) synchronized identification phase, (iii) update phase, (iv) desynchronized identification phase, (v) controlled delegation phase, (vi) owner transfer phase, and (vii) authorization recovery. Tables~\ref{tab:Protocolo} and~\ref{tab:other_phases} depict all these algorithms excepting both initialization and authorization recovery phases.

\subsubsection{Initialization}

Two unique keys, $ik$ and $uk$, are generated for each tag. Then, $ik$, $uk$
and $id$ are written on the non-volatile memory of the tag via a
secure channel. This information will be used later by the tag to
perform identification and ownership transfer.
After tag initialization, the server stores the tag
data in its database (see Table \ref{tab:Tabla-de-valores}).


\subsubsection{Synchronized identification phase}

When the tags are synchronized, they execute this phase in order
to be identified by a legitimate reader.
\begin{enumerate}
\item First, the reader broadcasts
a nonce $r_0$.
\item Then, the synchronized tag answers with the following
information: $h_{id}(ik)$, $C_0=PRNG(ik||r_0||r_1)$\footnote{The
pseudo-random number generator PRNG is supposed to be secure and
unpredictable.} and $r_1$. After sending all data, the tag switches
to a desynchronized state ($SYNC=0$) until the update phase ends.
\item Upon reception of these data, the reader forwards them to the server.
\item Then, the server searches inside a lookup table
the value $h_{id}(ik)$ and obtains the tag's data $ik$ and $id$.
Using the identification key $ik$ and the nonces $r_0$ and $r_1$,
the server checks $C_0$ and decides whether to send $id$ to the reader.
Note that by checking $C_0$ the server avoids phishing or replay attacks.
Finally, the server saves $r_0$ and $r_1$. These values are used
in the update phase.
\end{enumerate}

\subsubsection{Update phase}

All the features of our protocol are mainly based on this phase.
\begin{enumerate}
\item The server composes $m$ by concatenating a new
identification key $m_L=ik_{new}$ and its hash value
$m_R=h_{id}(ik_{new})$. Finally, the server computes
$C_1=m\oplus S$ where $S = PRNG(h_{uk}(ik)||id||r_0||r_1)$ is an
unpredictable pseudorandom sequence.
The server sends $C_1$ to the
reader.
\item The reader forwards $C_1$ to the tag.
\item Upon reception
of $C_1$, the tag generates its own pseudorandom
sequence $S' = PRNG(h_{uk}(ik)||id||r_0||r_1)$,
and computes $m'=C_1 \oplus S'$. By splitting $m'$,
the tag obtains $m_R'$ and $m_L'$ and checks whether
$m_R' = h_{uk}(m_L')$. If so, the tag can be sure that $m'$ is, indeed,
$m$; otherwise the tag rejects the reader's response.
After the reader authentication, the tag
splits $m$ and updates its data: $ik = m_L'$, $\delta = 0$ and $SYNC = 1$.
\end{enumerate}

\subsubsection{Desynchronized identification phase}

This phase is executed when reader and tag are desynchronized,
{\em e.g.} the message $C_1$ corresponding to the update
phase was incorrect or it had not been received. The steps are as follows:
\begin{enumerate}
\item The reader sends $r_0$ to the tag, like in the synchronized
identification phase.
\item The tag generates a new nonce $r_1$ and
computes: \newline $\delta=\delta+1$, $k_{\delta}=h_{uk}(k_{\delta-1})$ where $k_0=h_{id}(ik)$, and $C_0 = PRNG(k_{\delta+1}||id||r_0||r_1)$.
Finally, the tag sends $k_{\delta}$ and $C_0$ to the reader and stores the value $k_{\delta}$ for the next desynchronized identification phase if needed.
\item Upon reception of the tag's response, the reader forwards the
data to the server, who will search the value $k_{\delta}$
in the database using a lookup table generated with all
the $Table\, k$ in the database
(see Table \ref{tab:Tabla-de-valores}).
If the $k_{\delta}$ value is not found, the identification process
fails. Otherwise, if $k_{\delta}$  is found in one or more records
of the database, the server obtains the correct identifier
through search of the $id$ matching the $C_{0}$ value.
\item After a correct identification
of the tag, the reader starts the Update phase.
\end{enumerate}

It should be remarked that, the desynchronized identification
phase can be executed consecutively just $MAX$ times.
If the number of consecutive identifications by a desynchronized
identification phase is greater than $MAX$, the server
will not be able to identify the tag any more (denial of service).
The value of the parameter $MAX$ is extensively discussed
in~\cite{FernandezCV-2010-setop}.

%------------------------
\begin{table}[!ht]
\caption{Our protocol}
\label{tab:Protocolo}
\resizebox{\textwidth}{!}{
\begin{tabular}{>{\centering}m{0.43\paperwidth}>{\centering}m{0.2\paperwidth}>{\centering}m{0.2\paperwidth}}
\toprule
~
\begin{tabular}{>{\centering}m{0.19\paperwidth}>{\centering}m{0.20\paperwidth}}
\raggedright{}\textbf{Server} & \raggedleft{}\textbf{Reader}\tabularnewline
\end{tabular} &  & ~
\textbf{Tag}
\tabularnewline \tabularnewline
\multicolumn{3}{l}{\emph{Initialization phase (with secure channel)}}\\
\hline
\raggedleft{} & $ik, uk, id$\\
\begin{picture}(70,0)
\put (0,0){\vector(1,0){70}}
\end{picture} & \tabularnewline \tabularnewline
\multicolumn{3}{l}{\emph{Synchronized identification phase}}\\
\hline
\raggedleft{}$r_{0}\in{R}\{0,1\}^{*}$ & $r_{0}$\\
\begin{picture}(70,0)
\put (0,0){\vector(1,0){70}}
\end{picture} & \tabularnewline
 &  & \begin{raggedright}
$r_{1}\in{R}\{0,1\}^{*}$
\par\end{raggedright}
\begin{raggedright}
$C_{0}=PRNG(ik||r_{0}||r_{1})$
\par\end{raggedright}
\begin{raggedright}
Computes $h_{id}(ik)$
\par\end{raggedright}
\raggedright{}$SYNC=0$\tabularnewline
$h_{id}(ik),C_{0},r_{1},r_{0}$\\
\begin{picture}(70,0)
\put (70,0){\vector(-1,0){70}}
\end{picture} & $h_{id}(ik),C_{0},r_{1}$\\
\begin{picture}(70,0)
\put (70,0){\vector(-1,0){70}}
\end{picture} & \tabularnewline
\begin{raggedright}
Searches $h_{id}(ik)$
\par\end{raggedright}
\raggedright{}Checks $C_{0}$ &  & \tabularnewline \tabularnewline
\multicolumn{3}{l}{\emph{Update phase}}\\
\hline
\begin{raggedright}
$m_{L}=uk_{new}, \, m_{R}=h_{uk}(ik_{new})$
\par\end{raggedright}
\begin{raggedright}
$m=m_{L}||m_{R}$
\par\end{raggedright}
\begin{raggedright}
$S=PRNG(h_{uk}(i_k)||id||r_{0}||r_{1})$
\par\end{raggedright}
\raggedright{}$C_{1}=m\oplus S$ &  & \tabularnewline
$C_{1}$\\
\begin{picture}(70,0)
\put (0,0){\vector(1,0){70}}
\end{picture} & $C_{1}$\\
\begin{picture}(70,0)
\put (0,0){\vector(1,0){70}}
\end{picture} & \tabularnewline
 &  & \begin{raggedright}
$S^{'}=PRNG(h_{uk}(i_k)||id||r_{0}||r_{1})$
\par\end{raggedright}
\begin{raggedright}
$m^{'}=C_{1}\oplus S^{'}$
\par\end{raggedright}
\begin{raggedright}
$m^{'}_{R}\stackrel{?}{=}h_{uk}(m^{'}_{L})$
\par\end{raggedright}
\begin{raggedright}
$ik=m^{'}_{L}$
\par\end{raggedright}
\raggedright{}$SYNC=1$
\begin{raggedright}
$\delta=0$
\par\end{raggedright}
\tabularnewline \tabularnewline
\multicolumn{3}{l}{\emph{Desynchronized identification phase}}\\
\hline
\raggedleft{}$r_{0}\in{R}\{0,1\}^{*}$ & $r_{0}$\\
\begin{picture}(70,0)
\put (0,0){\vector(1,0){70}}
\end{picture} & \tabularnewline
 &  & \begin{raggedright}
$r_{1}\in{R}\{0,1\}^{*}$
\par\end{raggedright}
\begin{raggedright}
$k_{0}=h_{id}(ik)$
\par\end{raggedright}
\begin{raggedright}
$\delta=\delta+1$
\par\end{raggedright}
\begin{raggedright}
$k_{\delta}=h_{uk}(k_{\delta-1})$
\par\end{raggedright}
\raggedright{}$C_{0}=PRNG(k_{\delta+1}||id||r_0||r_1)$ \tabularnewline
$k_{\delta},C_{0},r_{1}$\\
\begin{picture}(70,0)
\put (70,0){\vector(-1,0){70}}
\end{picture} & $k_{\delta},C_{0},r_{1}$\\
\begin{picture}(70,0)
\put (70,0){\vector(-1,0){70}}
\end{picture} & \tabularnewline
\begin{raggedright}
Searches $k_{\delta}$ on $Table\, k$.
\par\end{raggedright}
\begin{raggedright}
Checks $C_{0}$
\par\end{raggedright}
\raggedright{}Start update phase &  & \tabularnewline
\tabularnewline
\bottomrule
\end{tabular}
}
\end{table}
\begin{center}
%

\par\end{center}

\subsubsection{Controlled delegation phase}

This phase is run when the current owner needs to delegate
identification rights to a new reader.
\begin{enumerate}
\item First, the current owner
runs a successful synchronized identification phase but skips
the update phase. At this stage, the tag is desynchronized and
therefore responds with $k_{\delta}$ values when queried.
\item Then, the current owner just needs to give to the new reader
the following infomation: $id$ and $n$ values of
$k_{\delta}$.
\item Later, the current owner is able to recover full control over
the tag using one of the two following strategies: i) run
a successful synchronized identification phase together with an
update phase or ii) query the tag $n$ times where $n$ is the
number of values given to the new reader.
\end{enumerate}
When the new reader identifies a tag $n$ times by controlled delegation, loose the right to identify this tag and only the current owner is able to identify the tag again. If the new reader needs to identify this tag again, it must request authorization to the current owner one more time

%------------------------

\subsubsection{Owner transfer phase.}

This phase is used to transfer ownership of the tag from the
current owner to the new owner. The basic idea is to use
a temporary key, as shown in Figure~\ref{fig:update}.

\begin{enumerate}
\item First, the current owner updates the key $uk$ with $uk_{tmp}$.
This prevents the new owner from backward tracking the tag.
\item Next, the current owner gives to the new owner the key $uk_{tmp}$.
\item Finally,  the new owner updates $uk_{tmp}$ with $uk_{new}$
to prevent the old owner from forward tracking the tag.
\end{enumerate}

After the previous protocol,
the current owner plays the role of the previous owner
while the new owner becomes the current owner. It should be remarked
that a tag can know that $uk$ is being updated by
computing the left part of  $C_2$. On the other hand, the new owner
should update $uk$ in an isolated environment in order to prevent the current
owner from eavesdropping the messages and computing $uk_{new}$.

\begin{figure}
  \centering
$uk
\longrightarrow
uk_{tmp}
\longrightarrow
uk_{new}$
\caption{\label{fig:update} Life-cycle of the update key
during the ownership transfer process}
\end{figure}


\subsubsection{authorization recovery}

In our scheme, an authorization recovery process can be performed
as a controlled delegation process. However, we must assume
that the current owner is unwilling to give the tag's
identifier to another reader.  The previous owner must search
in its data base an identifier that matches $C_0$ using one of the
provided values $(k_{\delta}$. Note that
this checking process can be only performed by a previous owner of a tag
and, hence, the tag can be identified only by a legitimate
previous owner.

%-----------------------------------


\begin{center}
\begin{table}[!ht]
\caption{Controlled delegation
and owner transfer phases}
\label{tab:other_phases}
\begin{tabular}{lcccr}
\toprule
\textbf{Current User} &  & \textbf{Tag} &  & \textbf{Final User}\tabularnewline\tabularnewline
%%%Controlled delegation
\multicolumn{5}{>{\raggedright}p{1\columnwidth}}{\emph{Controlled delegation phase}}
\\
\hline
\tabularnewline
\multicolumn{3}{c}{Synchronized identification phase}\\
\begin{picture}(150,0)
\put (50,0){\vector(1,0){150}}
\end{picture}
&  & \tabularnewline
 &  & $SYNC=0$ &  & \tabularnewline\tabularnewline
\multicolumn{5}{c}{\begin{tabular}{c}
$id$ and $n$ values of $k_{\delta}$ (with secure channel)\\
\begin{picture}(270,0)
\put (0,0){\vector(1,0){270}}
\end{picture}
\tabularnewline
\end{tabular}}\tabularnewline\tabularnewline
 &  & \multicolumn{3}{r}{Desynchronized identification phase}
 \\
 \begin{picture}(130,0)
\put (332,0){\vector(-1,0){130}}
\end{picture}
 \tabularnewline
 &  & $SYNC=0$ &  & \tabularnewline\tabularnewline
%%%Owner transfer
\multicolumn{5}{>{\raggedright}p{1\columnwidth}}{\emph{Owner transfer phase}}
\\
\hline
\tabularnewline
\begin{raggedright}
$m_{L}=uk_{new}, \, m_{R}=h_{uk}(uk_{new})$
\par\end{raggedright}
\tabularnewline
\begin{raggedright}
$m=m_{L}||m_{R}$
\par\end{raggedright}
\tabularnewline
\begin{raggedright}
$S=PRNG(h_{uk}(i_k)||id||r_{0}||r_{1})$
\par\end{raggedright}
\tabularnewline
\begin{raggedright}
$C_{2}=m\oplus S$
\par\end{raggedright}
 &  &  &  &
\tabularnewline
\multicolumn{3}{c}{$C_2$}\\
\begin{picture}(150,0)
\put (50,0){\vector(1,0){150}}
\end{picture}
&  &
\tabularnewline
 &  &
\begin{tabular}{l}
$S^{'}=PRNG(h_{uk}(i_k)||id||r_{0}||r_{1})$ \tabularnewline
$m^{'}=C_{2}\oplus S^{'}$ \tabularnewline
$m^{'}_{R}\stackrel{?}{=}h_{uk}(m^{'}_{L})$ \tabularnewline
$uk=m^{'}_{L}$
\end{tabular}
 &  & \tabularnewline\tabularnewline
\multicolumn{5}{c}{\begin{tabular}{c}
all data of the tag (with secure channel)\\
\begin{picture}(270,0)
\put (0,0){\vector(1,0){270}}
\end{picture}
\tabularnewline
\end{tabular}}\tabularnewline\tabularnewline
 &  & \multicolumn{3}{c}{\ \ \ \ \ \ \ \ \ \ Owner transfer phase}
 \\
 \begin{picture}(130,0)
\put (332,0){\vector(-1,0){130}}
\end{picture}
 \tabularnewline
 %%%%%%%%%%%%%%%%%%%%
\bottomrule
\end{tabular}
\end{table}
\end{center}






\subsection{Protocol states}

In this protocol, a tag can be in one of the following states: initialized,
synchronized, desynchronized and owner transfer. The tag changes
its state by means of the following operations:

\begin{itemize}
 \item (a) Initializing a tag. Once a tag has been initialized,
 it goes to the synchronized state.
 \item (b) Identifying a tag when it is synchronized. Once the tag is
 synchronized, if an identification is requested then its state
 changes to desynchronized.
 \item (c) Updating a tag. After a tag has been identified,
 the reader sends an update message. If the message is verified
 properly by the tag, the tag goes to the synchronized state.
 \item (d) Identifying a tag when it is desynchronized
 does not change the tag's state. Thus, the tag will remain desynchronized.
 \item (e) Running an owner transfer protocol. When the current owner
runs the owner transfer phase, the tag changes its state to owner transfer.
When the operation is verified successfully, the tags state is set to
synchronized.
 \item (f) Disabling a tag. If the desynchronized identification
 phase is run more than $MAX$ consecutive times, the tag is disabled
 (denial of service).
\end{itemize}


Figure \ref{fig:stats} shows the different states and operations that are possible in the protocol.

\begin{figure}
  \centering
   \includegraphics[scale=0.35]{ownership_figures/stats.pdf}
  \caption{The state diagram contains the states and
  transitions of an RFID tag in our scheme. The states
  are the following: i) tag initialized (INIT), ii) tag
  synchronized (SYNC), iii) tag desynchronized (DSYNC), and iv)
  tag disabled (DoS).}
  \label{fig:stats}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Analysis}
\label{analisis}
The protocol has the following security and privacy properties.

\subsection{Privacy}

We consider the following privacy property:

  \subsubsection{Monitoring and location.}
  Location privacy is guaranteed because, in each identification,
  the data sent are always different,
  thanks to the use of nonces $r_0$ and $r_1$.
 Indeed,
  values $ik$, $h_{id}(ik)$, $C_0$ and $r_1$ are updated in each identification.
If the reader and the tag are not synchronized, then the updated elements are: $k_\delta$, $C_0$ and $r_1$.
  If both devices are synchronized, $h_{id}(ik)$ can appear twice with a probability of $1/2^{\ell}$ where $\ell$ is the size of the hash function.

 The probability for $k_\delta$ is the same as $h_{id}(ik)$ in
  consecutive secondary identifications.

\subsection{Security}

Below are the most common attacks which can be launched on RFID schemes:

  \subsubsection{Denial of service.}

  An attacker can query the tag or interrupt the update phase $MAX+1$ times,
  so that after that,
  a legitimate reader will not find $k_{\delta}$ in the database
  and will not be able to identify the tag. Since
  $MAX$ is a security parameter of our system, we can set this value
  in order to increase the resistance of the proposed protocol
  against this attack.
  If the table is large enough, the time needed to consume all the
  values will be high enough. For instance, for $MAX=100,000$
  the required time to obtain all values of $Table\, k$ by an attacker,
  taking into account that each identification needs an interval of 200 ms, is 5.5 hours. By contrast, the disk space needed in a system with only 100,000 tags is 24 Tb.

  To prevent massive attacks, the system can identify the tags regurarly. In this case, if an attacker is trying to knock out a tag, once the system updates that tag, the attacker must restart the DoS attack from zero. Furthermore, the value of $MAX$ can be parameterized to resist DoS attacks.
  The fact that a high value of $MAX$ behave a high space in disk is assumed due to the low cost of storage units today, yet this is one aspect to improve in a future versions of this protocol.



  \subsubsection{Impersonation of devices.}

  \begin{itemize}

  \item \emph{Impersonating a certain tag.}
  An attacker does not know values $ik$, $uk$ and $id$. These elements
  are sent in the initialization phase using a secure communication channel.
  An attacker trying to impersonate a certain tag without the knowledge
  of these values will be detected by the reader. If an attacker
  is able to obtain the tag values, this information does not
  compromise other tags.
Hence, impersonating a tag requires physically tampering with it and,
in that case, it allows impersonating only that tag.

  \item \emph{Impersonating the server.}
  This case is similar to the previous property.
  The server can only be impersonated by an attacker who
  knows the entire database. We assume that the database is
  hosted in a secure environment.

  \item \emph{Replay attacks.}
  This type of attack is not possible in this protocol because,
  in each identification, each of the sides (tag and server) provides
  a new value which is computed at random. In this way, a replay attack
  at the server side will be successful only if the message which
  has been captured previously contains the expected $r_0$ value.
  The same happens at the tag side but with the value $r_1$.
  Random nonces $r_0$ and $r_1$ are generated in
  each device and they are unlikely to be repeated over
  a short period of time. In this way, value $h_{id}(ik)$ is
  different in each synchronized identification phase. In
  the desynchronized identification phase case, $k_\delta$ is always different.

	\end{itemize}

\subsection{Ownership transfer}

Our proposal satisfies the following properties.

  \subsubsection{New owner privacy} Our protocol is designed to
  guarantee that the transactions between the
  current owner and the tag cannot be traced by the previous owner.
  When the ownership of the tag is transferred, $uk$ and $ik$ are
  randomly updated, thereby ensuring that previous owners cannot
  identify the tag anymore unless the current owner allows
  controlled delegation.

  \subsubsection{Previous owner privacy} Since the update key is changed
  twice ($uk \rightarrow uk_{tmp} \rightarrow ik$), the previous owner's
  privacy is also guaranteed. As a result, the current owner cannot trace
  previous transactions between the previous owner and the tag.

  \subsubsection{authorization recovery} The protocol satisfies
  this property because the current owner can delegate the
  reading of the tag in a controlled fashion.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}
\label{conclusions}

The novelty of our proposal consists of leveraging the update phase,
which is used in the RFID identification protocol, in order to implement
the ownership transfer protocol. Moreover, the protocol allows
controlled delegation without the need of a counter in the
non-volatile memory of tags. This feature is especially important
considering that: i) tags are resource-constrained devices;
ii) readers should not share the identification key of a tag.
Finally, the protocol does not need a TTP, so that the users can perform
ownership transfers any time and anywhere.






